From Deep Learning to LLMs: A survey of AI in Quantitative Investment

Quantitative investment (quant) is an emerging, technology-driven approach in asset management, increasingy shaped by advancements in artificial intelligence. Recent advances in deep learning and large language models (LLMs) for quant finance have improved predictive modeling and enabled agent-based automation, suggesting a potential paradigm shift in this field. In this survey, taking alpha strategy as a representative example, we explore how AI contributes to the quantitative investment pipeline. We first examine the early stage of quant research, centered on human-crafted features and traditional statistical models with an established alpha pipeline. We then discuss the rise of deep learning, which enabled scalable modeling across the entire pipeline from data processing to order execution. Building on this, we highlight the emerging role of LLMs in extending AI beyond prediction, empowering autonomous agents to process unstructured data, generate alphas, and support self-iterative workflows.

==> discussion.tex <==
\section{Open Problems and Future Directions}
After introducing the roadmap of AI investment engineering from both algorithm and system perspectives, we summarize the open problems that remain to be solved and some promising research directions.

\subsection{The Gap between Academia and Industry Applications}
The gap between academia and industry is  significant for quantitative investment. The research community mainly focuses on some well-established tasks such as stock prediction and portfolio optimization \cite{jiang_applications_2021, hu_survey_2021, thakkar_comprehensive_2021, zhang_deep_2020}. However, the industry cares more about the whole quantitative workflow as the improvement in a single component may not generalize to the whole system. 
% Problem in other parts of the pipeline, such as risk management using deep learning, are not actively studied by the machine learning research community. 
Studying how to optimize a quantitative investment system in an end-to-end manner is therefore a promising research direction academia.

% These features induce the fundamental problems to be solved. As discussed in Section \ref{sec:introduction}, the low SNR increases the difficulty of learning meaningful patterns. The high volatility makes the trained model deteriorate soon or even invalidates the performance verification based on backtest since we cannot make sure the same performance on history data can be reproduced on the data from new distributions. Moreover, the multi-modality and ubiquity of financial-related data complicates the modelling process. It is often the case that we have abundant data at hand while lacking powerful tools to analyze them and make better predictions.

\subsection{Lack of Specialized Algorithms for Quantitative Investment}
Quantitative investment has some significant characteristics that differentiate it from the other machine learning problems: (1) low signal-to-noise ratios in data; (2) non-stationary distributions given the dynamic nature of the financial markets; (3) incomplete information. The performance of most machine learning models deteriorates in financial applications. Hence, we advocate specialized algorithms for quantitative investment. On the other hand, many recent advances in the machine learning community have not been transferred to quantitative investment, e.g.\ efficient learning on heterogeneous tabular data \cite{borisov_deep_2021}, continual/incremental learning \cite{de_lange_continual_2022}, large-scale pre-trained models \cite{bommasani_opportunities_2021}.


%Therefore, we expect that the comprehensive combination of state-of-the-art AI techniques and a wider range of quantitative investment tasks should be a future trend in this research field. On one hand, more quantitative investment tasks needs to be studied from AI's perspective. On the other hand, the abundant research progress in DL field such as contrastive learning, multi-modal learning and large-scale pretraining also needs to be applied to quantitative investment researches.
% The  of quantitative investment systems has two major trends: to become bigger and become faster. Becoming bigger requires the scalability of the system to be improved, which involves 

% researches in distributed systems and parallel computing. Becoming faster, on the other hand, requites reducing the latency of the system, which involves algorithmic improvements as well as the hardware-software co-design of the trading system.
\subsection{Lack of Well-Established Quantitative Investment Systems}
The progress of quantitative investment relies on rigorous engineering practice. However, there are few open-sourced quantitative investment systems, which impedes the research progress on quantitative investment systems. Following the discussion in \S\ref{sec:quant_system}, we advocate the research on designing quantitative investment systems that have high concurrency, high scalability, and low latency.

\subsection{Reproducibility Crisis}
Although there have been many public machine learning frameworks for quantitative investment \cite{yang_qlib_2020, freitas_awesome-quant_2022}, one major challenge for the research community is that research works adopt different data preprocessing, evaluation methods, and datasets, which hurts the reproducibility of the research works. Unlike other fields such as NLP and computer vision \cite{wang_glue_2019, deng_imagenet_2009, lin_microsoft_2014}, the quantitative investment research community does not have a well-established benchmark to compare different algorithms and monitor the research progress. It is essential to build such benchmarks to facilitate rigorous research practice. 

%the inconsistency among research papers, which can be instantiated as the difference in evaluating protocols, datasets and the incorrectness in evaluation methods. The main reason for such a situation is the lack of consistent framework for benchmarking and evaluating various research works for the community, which is common practice in CV and NLP.

%The framework are expected to provide unified data sources and evaluation protocols to guarantee consistency, implement correct evaluation methods and metrics for correctness, and open-sourcing the implementations of some famous and classical algorithms for convenient re-producing and benchmarking novel methods. Such a framework can pave the way for future researches and have profound impact on the developing of this rising field.
